Anomalous transport coefficients from Kubo formulas in Holography

In the presence of dense matter quantum anomalies give rise to two new transport phenomena. An anomalous current is generated either by an external magnetic field or through vortices in the fluid carrying the anomalous charge. The associated transport coefficients are the anomalous magnetic and vortical conductivities. Whereas a Kubo formula for the anomalous magnetic conductivity is well known we develop a new Kubo type formula that allows the calculation of the vortical conductivity through a two point function of the anomalous current and the momentum density. We also point out that the anomalous vortical conductivity can be understood as a response to a gravitomagnetic field. We apply these Kubo formulas to a simple Holographic system, the R-charged black hole.

==> T0.tex <==
%\section{Anomalous transport at $T=0$}

==> w-diff-0.tex <==
\section{Computation at $\omega\neq0$}\label{wdiff0}

As we analyzed, in the hydrodynamic regime the velocity of the ßuid in de Landau 
frame is determined modulo a P -odd term $v_m\sim\frac{\partial_x^3}{(\epsilon+P)\partial_t-\eta\partial_x^2}f(t,x)$ with $f(t,x)$ an 
arbitrary function of the sources, this appendix pretends realize holographically this 
ambiguity, show the independence of the transport coe?cients on this arbitrary func- 
tion and demonstrate that our deÞnition for ?V (?) and ?B (?) are are well deÞned 
functions. 
The system \ref{constraint}-\ref{bx} can be simpliÞed if we redeÞne hit as 
\be
h^i_t (u) = \tilde h^i_t +\int_0^u  h^i_{tp} (m)\textrm dm + 3a \int_0^u mB_i (m)\textrm dm,
\ee
this new field has the particularity that $h'^i_t (0) = h^i_{tp}(0)$ 

